Decentralized Consensus Optimization with Asynchrony and Delays

We propose an asynchronous, decentralized algorithm for consensus optimization. The algorithm runs over a network in which the agents communicate with their neighbors and perform local computation. In the proposed algorithm, each agent can compute and communicate independently at different times, for different durations, with the information it has even if the latest information from its neighbors is not yet available. Such an asynchronous algorithm reduces the time that agents would otherwise waste idle because of communication delays or because their neighbors are slower. It also eliminates the need for a global clock for synchronization. Mathematically, the algorithm involves both primal and dual variables, uses fixed step-size parameters, and provably converges to the exact solution under a bounded delay assumption and a random agent assumption. When running synchronously, the algorithm performs just as well as existing competitive synchronous algorithms such as PG-EXTRA, which diverges without synchronization. Numerical experiments confirm the theoretical findings and illustrate the performance of the proposed algorithm.

==> shortanalysis.tex <==
We present our main assumptions and convergence results. As space is limited, all proofs are left to the longer report.



\begin{assumption}\label{assum:random}
For any $k>0$, the index $i_k$ of the agent responsible for the $k$th update is random and has probability $$q_i:=P(i_k=i)>0.$$
The random variables $i_1,i_2,\cdots$ are independent.
\end{assumption}
This assumption is satisfied under either of the following scenarios: (i) every agent $i$ is activated following an independent Poisson process with parameter $\lambda_i$ and its computation is instant, leading to $q_i = \lambda_i / (\sum_{i=1}^n \lambda_i)$; (ii) every agent $i$ runs continuously, and the duration of each round follows the exponential distribution $\exp(\beta_i)$, leading to $q_i=\beta_i^{-1} / (\sum_{i=1}^n \beta_i^{-1})$. Scenarios (i) and (ii) appear in some literature as assumptions. 
%This alternative assumption implies that the activation of any agent is a Poisson process with the parameter $\sum_{i=1}^n\lambda_i$, and the agent activated is random, independent of previous activations. Assumption~\ref{assum:random} also holds if each agent $i$ computes continuously and its computation time follows the exponential distribution with a parameter $\lambda_i$ (denoted by exp$(\lambda_i)$).
%In a real-life network, since each agent computes and passes data non-stop, the delay caused by the computation and communication time should have an upper bound. Even when there exists some packet loss, the subsequent packets will catch up and keep the delay in a relatively low level. We make this explicit:
\begin{assumption}
The delays $\tau_j^k,j=1,2,\ldots,n$ and $\delta_e^k,e=1,2,\ldots,m$, $\forall k$, defined in~\eqref{update_asyn} have an upper bound $\tau>0$.
\end{assumption}
Since the weight matrix $W$ associated with the network is symmetric and doubly stochastic, its eigenvalues lie in $[-1,1]$. We further restrict its minimum eigenvalue $\lambda_{\min}(W)$:
\begin{assumption}\label{eigenassum}
$\lambda_{\min}(W)>-1$.
\end{assumption}
%An important consequence of this assumption is:  %($I$ is the identity operator):
%(recall $V^\top V=\frac{1}{2}(I-W)$):
\begin{lemma}
Under Assumption~\ref{eigenassum}, we have 
\begin{equation}\label{metric}
G:=\begin{bmatrix}
I&V^\top\\
V&I
\end{bmatrix}\succ \vzero.
\end{equation} %is positive definite.
\end{lemma}
Let $\rho_{\min}:=\lambda_{\min}(G)>0$ be the smallest eigenvalue of $G$ and $\kappa$ be its condition number. 
%We make assumptions on the functions $s_i$ and $r_i$, and the parameter $\alpha$.
\begin{assumption}\label{assumfunc}
$ $
\begin{enumerate}
\item The functions $s_i$ and $r_i$ are closed, proper and convex;
\item the functions $s_i$ are differentiable and satisfy:
$$\|\nabla s_i(x)-\nabla s_i(\tilde{x})\|\leq L_i\|x-\tilde{x}\|,\quad\forall x,\tilde{x}\in\RR^p;$$
\item the parameter $\alpha$ in Eq.~\eqref{alg:cv2} and Alg.~\ref{alg:asyn} satisfies $0<\alpha<\frac{2\rho_{\min}}{L}$, where $L=\max_i L_i$.
\end{enumerate}
\end{assumption}
We have the following theorem for $\vz^k:=[\vx^k;\vy^k]$.
\begin{theorem}\label{thm:async-convergence2}
Let $Z^*$ be the set of primal-dual solutions to~\eqref{prob:saddle}, $(\vz^k)_{k\geq0}$ be the sequence generated by Alg.~\ref{alg:asyn}, and $\eta_i
\in (0, \eta_{\max}]$ where $\eta_{\max}<\frac{nq_{\min}}{2\tau
\sqrt{\kappa q_{\min}}+\kappa}$ and $q_{\min}:=\min_i q_i$.
Then $(\vz^k)_{k\geq 0}$ converges to a point in $Z^*$ with probability 1.
\end{theorem}
This theorem guarantees that, if we run the asynchronous algorithm~\ref{alg:asyn} from an arbitrary starting point $\vx^0$, then with probability $1$, the sequence $\{\vx^k\}$ produced will converge to one of the solutions to problem~\eqref{prob:saddle}. The upper bound of $\eta_{\max}$ becomes smaller if the maximum delay is larger, or if the matrix $M$ becomes more ill-conditioned. While the theorem bounds $\eta_i$ by a uniform $\eta_{\max}$, the bound can be improved by locally adapting it  to the delay only pertaining to agent $i$. We leave this and other improvements to the longer report.
%\commtw{Actually, shall we briefly introduce monotone operator theory at the beginning? We need at least define the proximal operator.}

